The impact of the spatial resolution of wind data on multi-decadal wind power forecasts in Germany

Accurate multi-decadal wind power predictions are crucial for sustainable energy transitions but are challenged by the coarse spatial resolution of global climate models (GCMs). This study examines the impact of spatial resolution on wind power forecasts by analyzing historical wind speed outputs from ten CMIP6 GCMs in Germany, using ERA5 reanalysis as a reference. Results show that the choice of GCM is the primary influence on wind speed output, with higher resolution models partly, but not consistently, improving predictions. While high-resolution models better capture extreme wind speeds, they do not systematically improve the prediction of the whole wind speed distribution. The data set MPI-ESM1-2-HR (MPI-HR) was found to represent the wind speed distribution particularly faithfully, while the MIROC6 (JAP) data set showed substantial underestimation for the German region compared to ERA5. These findings underscore the complexity of wind speed modeling for power predictions and emphasize the need for careful GCM selection and appropriate downscaling and bias correction methods.

==> misc/abstract.tex <==
Accurate multi-decadal wind power predictions are crucial for sustainable energy transitions but are challenged by the coarse spatial resolution of global climate models (GCMs). This study examines the impact of spatial resolution on wind power forecasts by analyzing historical wind speed outputs from ten CMIP6 GCMs in Germany, using ERA5 reanalysis as a reference. Results show that the choice of GCM is the primary influence on wind speed output, with higher resolution models partly, but not consistently, improving predictions. While high-resolution models better capture extreme wind speeds, they do not systematically improve the prediction of the whole wind speed distribution. The data set MPI-ESM1-2-HR (MPI-HR) was found to represent the wind speed distribution particularly faithfully, while the MIROC6 (JAP) data set showed substantial underestimation for the German region compared to ERA5. These findings underscore the complexity of wind speed modeling for power predictions and emphasize the need for careful GCM selection and appropriate downscaling and bias correction methods. 

\subsubsection{Deutsche Version}
\textit{Genaue Vorhersagen der Windenergie über mehrere Dekaden hinweg sind für eine nachhaltige Energiewende von entscheidender Bedeutung, werden jedoch durch die grobe räumliche Auflösung globaler Klimamodelle (GCMs) erschwert. Diese Studie untersucht die Auswirkung der räumlichen Auflösung auf Windkraftprognosen durch die Analyse historischer Windgeschwindigkeitsdaten von zehn CMIP6-GCMs in Deutschland, wobei die ERA5-Reanalyse als Referenz dient. Die Ergebnisse zeigen, dass die Wahl des GCMs die Windgeschwindigkeit maßgeblich beeinflusst, wobei Modelle mit höherer Auflösung teilweise, aber nicht konsistent, die Vorhersagen verbessern. Während hochauflösende Modelle die extremen Windgeschwindigkeiten besser erfassen, verbessern sie nicht systematisch die Vorhersage der gesamten Windgeschwindigkeitsverteilung. Es wurde festgestellt, dass der Datensatz MPI-ESM1-2-HR (MPI-HR) die Windgeschwindigkeitsverteilung besonders genau wiedergibt,  während der Datensatz MIROC6 (JAP) die Windgeschwindigkeiten in der deutschen Region im Vergleich zu ERA5 erheblich unterschätzt. Diese Ergebnisse unterstreichen die Komplexität der Windgeschwindigkeitsmodellierung für Energievorhersagen und betonen die Notwendigkeit einer sorgfältigen GCM-Auswahl und geeigneter Downscaling- und Bias-Korrekturmethoden.}

